Neuro-Symbolic Program Synthesis

Recent years have seen the proposal of a number of neural architectures for the problem of Program Induction. Given a set of input-output examples, these architectures are able to learn mappings that generalize to new test inputs. While achieving impressive results, these approaches have a number of important limitations: (a) they are computationally expensive and hard to train, (b) a model has to be trained for each task (program) separately, and (c) it is hard to interpret or verify the correctness of the learnt mapping (as it is defined by a neural network). In this paper, we propose a novel technique, Neuro-Symbolic Program Synthesis, to overcome the above-mentioned problems. Once trained, our approach can automatically construct computer programs in a domain-specific language that are consistent with a set of input-output examples provided at test time. Our method is based on two novel neural modules. The first module, called the cross correlation I/O network, given a set of input-output examples, produces a continuous representation of the set of I/O examples. The second module, the Recursive-Reverse-Recursive Neural Network (R3NN), given the continuous representation of the examples, synthesizes a program by incrementally expanding partial programs. We demonstrate the effectiveness of our approach by applying it to the rich and complex domain of regular expression based string transformations. Experiments show that the R3NN model is not only able to construct programs from new input-output examples, but it is also able to construct new programs for tasks that it had never observed before during training.

==> background.tex <==

\section{Background}

We first present a brief overview of DSL-based synthesis approaches and then describe the subset of FlashFill DSL that we consider in this paper.

\subsection{DSL-based Synthesis}

The traditional formulation of program synthesis is to find a program that satisfies some correctness specification provided as a logical formula.  Instead of considering Turing complete languages as the hypothesis space of programs, a recent trend in a lot of program synthesis work has been to consider a syntactic restriction on the space of valid programs by designing a domain-specific language (DSL) -- also known as syntax-guided synthesis~\cite{sygus}. The DSL is designed to be expressive enough to encode a majority of the desired tasks in a domain, but at the same time designed to be concise enough for amenable learning. This syntactic restriction on the hypothesis space serves two purposes: i) it makes the search space more structured and tractable (although it is still often infinite), and ii) the learnt programs are interpretable as they correspond to derivations in the DSL. This approach has been used for many synthesis tasks including synthesizing low-level bitvector implementations~\cite{pldi05}, Excel macros for data manipulation~\cite{popl11,cacm12}, superoptimization by finding smaller equivalent loop bodies~\cite{stoke}, protocol synthesis from example scenarios~\cite{transit}, synthesis of loop-free programs~\cite{loopfree}, and automated feedback generation for programming assignments~\cite{autograder}.

The DSL is typically defined using a context-free grammar $G$. Given a logical specification $\spec$ (in the form of examples, partial constraints, reference implementation etc.), the computational synthesis problem is to find a derivation $f \in L(G)$ such that $f$ statisfies the specification $\spec$, where $L(G)$ denotes the language of the grammar. Several synthesis strategies have been developed for solving this computational problem, some of which include enumerative~\cite{transit}, stochastic~\cite{stoke}, symbolic~\cite{sketch,cvcsygus}, and version-space algebra~\cite{cacm12}.

The smart enumerative techniques have been shown to one of the most effective synthesis algorithms for learning small programs in rich complex hypothesis spaces~\cite{syguscompetition}. The main idea of these techniques is to first structure the hypothesis space using some measures such as program size, complexity etc., and then enumerate programs in the structured space with pruning to efficiently search for a program that satisfies the specification. The enumerative algorithms are typically designed to be semi-decidable for infinite hypothesis spaces, but they are also generally applicable for other kinds of hypothesis spaces and specification constraints.

We now describe a simple enumerative synthesis algorithm for hypothesis spaces that are defined using a CFG (similar to SyGuS~\cite{sygus}). Note that the algorithm can be easily extended to other forms of hypothesis spaces such as partial programs, context-sensitive languages etc. Let the hypothesis space be defined by a context-free grammar $G=(V,\Sigma,R,S)$, where $V$ denotes the set of non-terminals in the grammar, $\Sigma$ denotes a finite set of terminals including constants and program variables, $R$ denotes a finite relation from $V$ to $(V \cup \Sigma)^*$ corresponding to the grammar production rules, and $S$ denotes the start symbol. A simple grammar for defining the hypothesis space of a set of conditional linear arithmetic expressions over two variables \t{x} and \t{y} is shown in Figure~\ref{cliagrammar}.

\begin{figure}
\begin{lstlisting}[mathescape,numbers=none]
S $\rightarrow$ x | y | (S + S) | (S - S) | if(B,S,S)
B $\rightarrow$ (S $\leq$ S) | (S = S) | (S $\geq$ S)
\end{lstlisting}
\caption{A simple context-free grammar for defining a space of conditional linear integer arithmetic expressions.}
\label{cliagrammar}
\end{figure}


\begin{figure}
    \centering
    \small
    \begin{algorithmic}
        \Function{EnumSearch}{grammar $G$, spec $\spec$}
        	\State $\widetilde{P} \gets \{ S \}$ // Set of partial derivations in G
        	\While{$\widetilde{P} \neq \emptyset$}
        		\State $p \gets \Call{RemoveFirst}{\widetilde{P}}$
        		\If{$\phi(p)$} // Specification $\phi$ is satisfied
        			\State \Return $p$
        		\EndIf
        		\State $\widetilde{\alpha} \gets \Call{NonTerminals}{p}$
        		\ForEach {$\alpha \in \Call{RankNonTerminals}{\widetilde{\alpha},\spec}$}
        			\State $\widetilde{\beta} \gets \{(\alpha,\beta) | (\alpha, \beta) \in R\}$
        		\ForEach {$\beta \in \Call{RankProductionRule}{\widetilde{\beta},\spec}$}
        				\State $p' \gets p[\alpha \rightarrow \beta]$
        				\If{\Call{Subsumed}{$p',\widetilde{P},\spec$}}
	        				\State $\widetilde{P}.\Call{Insert}{p'}$
	        				\EndIf
        			\EndFor

        		\EndFor
        	\EndWhile
        \EndFunction
    \end{algorithmic}
    \caption{A simple enumeration algorithm to search for a derivation $p$ in a hypothesis space defined by a CFG $G$ that satisfies a given specification $\spec$.}
    \label{enumerativealgo}
    \end{figure}
    
A simple enumerative algorithm for searching over programs that satisfy a specification $\phi$ in a hypothesis space defined by a grammar $G$ is shown in Figure \ref{enumerativealgo}. The algorithm enumerates the derivations in the grammar starting from the start symbol $S$ in a top-down fashion and maintains an ordered set of partial derivations $\widetilde{P}$. It selects the first derivation $p$ from the set $\widetilde{P}$ and checks whether it satisfies the given specification $\phi$. If yes, the algorithm returns $p$ as the desired program. Otherwise, the algorithm computes the set of all non-terminal nodes $\widetilde{\alpha}$ in the partial derivation that can be expanded and ranks them using a pre-defined \textsc{RankNonTerminal} function. It then considers each non-terminal $\alpha$ in an ordered fashion and computes the set of possible production rules $\widetilde{\beta}$ for $\alpha$. The algorithm searches over the set of production rules again in a ranked order (using \textsc{RankProductionRule} function) to compute expanded derivations $p'$ where the non-terminal node $\alpha$ is replaced by $\beta$. Finally, the algorithm prunes the search space by avoiding adding a newly expanded program $p'$ if $p'$ is already subsumed by some program that has been previously considered by the algorithm. This algorithm iteratively continues until it finds a program $p$ satisfying the specification.



\subsubsection{FlashFill}

FlashFill, a recently introduced feature in Microsoft Excel 2013, is a Programming By Example (PBE) system for helping end-users perform string transformations using input-output examples. The key idea in FlashFill is to structure the hypothesis space of possible programs using an expressive and learnable DSL. It uses a version-space algebra based synthesis algorithm to efficiently learn programs in the DSL that are consistent with a given set of input-output examples. The syntax and semantics of a large subset of the FlashFill DSL (except conditionals) that we consider in this paper is shown in Figure~\ref{flashfilldsl}(a) and Figure~\ref{flashfilldsl}(b) respectively.


\begin{figure*}[!htpb]
\begin{tabular}{c|c}
\begin{minipage}{0.45\linewidth}

\begin{eqnarray*}
\mbox{String } e & := & \t{Concat}(f_1, \cdots, f_n) \nonumber \\
\mbox{Substring } f & := & \t{ConstStr}(s) \\
& | & \t{SubStr}(v,p_l,p_r) \nonumber \\
\mbox{Position } p & := & (r, k, \t{Dir}) \\
& | & \t{ConstPos}(k) \nonumber \\
\mbox{Direction } \t{Dir} & := & \t{Start} \; | \; \t{End} \nonumber \\
\mbox{Regex } r & := & s \; | \; T_1 \; \cdots \; | \; T_n
\end{eqnarray*}


\end{minipage}

&

\begin{minipage}{0.55\linewidth}

\begin{eqnarray*}
\sem{\t{Concat}(f_1,\cdots,f_n)} & = & \t{Concat}(\sem{f_1}, \cdots, \sem{f_n}) \\
\sem{\t{ConstStr}(s)} & = & s \\
\sem{\t{SubStr}(v,p_l,p_r)} & = & v[\sems{p_l}..\sems{p_r}]\\
\sem{\t{ConstPos}(k)} & = & k > 0 ? \; k : \t{len}(s)+k \\
\sem{(r,k,\t{Start})} & = & \mbox{Start of } k^{\t{th}} \mbox{match of r in v}\\
& &  \mbox{from beginning (end if } k<0 \mbox{)}\\
\sems{(r,k,\t{End})} & = & \mbox{End of } k^{\t{th}} \mbox{match of r in v}\\
& &  \mbox{from beginning (end if } k<0 \mbox{)}\\
\end{eqnarray*}
\end{minipage}

\\ \\
(a) & (b)
\end{tabular}
\caption{ The (a) syntax and (b) semantics of the FlashFill DSL we consider in this paper.}
\label{flashfilldsl}
\end{figure*}

A FlashFill program takes as input a string $v$ and returns an output string $o$. The top-level string expression $e$ is a concatenation of a finite list of substring expressions $f_1,\cdots,f_n$. A substring expression $f$ can either be a constant string $s$ or a substring expression, which is defined using two position logics $p_l$ (left) and $p_r$ (right). A position logic corresponds to a symbolic expression that evaluates to an index in the string. A position logic $p$ can either be a constant position $k$ or a token match expression $(r,k,\t{Dir})$, which denotes the \t{Start} or \t{End} of the $k^\t{th}$ match of token $r$ in input string $v$. A regex token can either be a constant string $s$ or one of 8 regular expression tokens: $p$ (ProperCase), $C$ (CAPS), $l$ (lowercase), $d$ (Digits), $\alpha$ (Alphabets), $\alpha n$ (Alphanumeric), $^\wedge$ (StartOfString), and \$ (EndOfString).


The semantics of the FlashFill programs is shown in Figure~\ref{flashfilldsl}(b). The semantics of a \t{Concat} expression is to concatenate the results of recursively evaluating the constituent substring expressions $f_i$. The semantics of \t{ConstStr(s)} is to simply return the constant string $s$. The semantics of a substring expression is to first evaluate the two position logics $p_l$ and $p_r$ to $p_1$ and $p_2$ respectively, and then return the substring corresponding to $v[p_1..p_2]$. We denote $s[i..j]$ to denote the substring of string $s$ starting at index i (inclusive) and ending at index j (exclusive), and \t{len}(s) denotes its length. The semantics of \t{ConstPos(k)} expression is to return $k$ if $k>0$ or return $\t{len}+k$ (if $k<0$). The semantics of position logic $(r,k,\t{Start})$ is to return the Start of $k^\t{th}$ match of r in $v$ from the beginning (if $k>0$) or from the end (if $k<0$).


An example FlashFill task is shown in Figure~\ref{namefirstlast}. The task requites to abbreviate a list of names to initials of first name and last names. A program in the FlashFill DSL that can perform this task is: \t{Concat}($f_1,\t{ConstStr(".")},f_2,\t{ConstStr(".")}$), where $f_1 \equiv \t{SubStr}(v,0,1)$ and $f_2 \equiv \t{SubStr}(v, (C,-1,\t{Start}), (C,-1,\t{End}))$. The program concatenates the following 4 strings: i) first character of the input string, ii) constant string \t{"."}, iii) substring between start of last capital token match and end of last capital token match, and iv) constant string \t{"."}.

\begin{figure}[!htpb]
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
& \multicolumn{1}{|c|}{\bf Input $v$} & \multicolumn{1}{|c|}{\bf Output} \\\hline\hline
1 & William Henry Charles & {\bf W.S.} \\ \hline
2 & Michael Johnson & {\bf M.J.} \\ \hline
3 & Barack Rogers & {\bf B.R.} \\ \hline
4 & Martha D. Saunders & {\bf M.S.} \\ \hline
5 & Peter T Gates & {\bf P.G.} \\ \hline
\end{tabular}
\end{center}
\caption{Abbreviating names to initials.}
\label{namefirstlast}
\end{figure}

